Motivo: fast motif counting via succinct color coding and adaptive sampling

The randomized technique of color coding is behind state-of-the-art algorithms for estimating graph motif counts. Those algorithms, however, are not yet capable of scaling well to very large graphs with billions of edges. In this paper we develop novel tools for the `motif counting via color coding' framework. As a result, our new algorithm, Motivo, is able to scale well to larger graphs while at the same time provide more accurate graphlet counts than ever before. This is achieved thanks to two types of improvements. First, we design new succinct data structures that support fast common color coding operations, and a biased coloring trick that trades accuracy versus running time and memory usage. These adaptations drastically reduce the time and memory requirements of color coding. Second, we develop an adaptive graphlet sampling strategy, based on a fractional set cover problem, that breaks the additive approximation barrier of standard sampling. This strategy gives multiplicative approximations for all graphlets at once, allowing us to count not only the most frequent graphlets but also extremely rare ones. To give an idea of the improvements, in $40$ minutes Motivo counts $7$-nodes motifs on a graph with $65$M nodes and $1.8$B edges; this is $30$ and $500$ times larger than the state of the art, respectively in terms of nodes and edges. On the accuracy side, in one hour Motivo produces accurate counts of $\approx \! 10.000$ distinct $8$-node motifs on graphs where state-of-the-art algorithms fail even to find the second most frequent motif. Our method requires just a high-end desktop machine. These results show how color coding can bring motif mining to the realm of truly massive graphs using only ordinary hardware.

==> related.tex <==
\section{Related work}
\label{sub:rel}
%The naive algorithm for counting the exact number of occurrences of all graphlets of size $k$ in an $n$-node graph by enumeration takes $O(k^2 n^k)$ time.
%Faster exact algorithms are known~\cite{Vassilevska&2013,Floderus&2015}, but their complexity remains $n^{\Theta(k)}$ and are infeasible in practice already for moderate values of $n$ and $k$.
Computing exactly the number of occurrences of a $k$-graphlet is hard, i.e.\ unlikely to admit algorithms substantially faster than $\Theta(n^k)$~\cite{Jerrum&2015}.
In practice, fast exact algorithms are known only for small values of $k$.
For $k=4$, the fastest method to date is the combinatorial technique of~\cite{Ahmed&2015}, which could process a graph on $n=148$M nodes in $25$ hours.
For $k=5$,~\cite{Pinar&2017} managed graphs on up to a few million nodes by exploiting a decomposition into smaller graphlets together with a degeneracy-like orientation of the graph -- the reported times vary from minutes to several days depending on the graph.
It is not clear how to extend those methods to $k>5$, even assuming the running time remains acceptable.

A more practical solution is to obtain \emph{approximate} graphlet counts.
There are different techniques used by approximate algorithms for graphlet counting:

\begin{itemize}
\item \textbf{Path sampling~\cite{Jha&2015}.} It consists in sampling graphlets by sampling their spanning trees, when those trees are paths.
This gives good results for $4$-graphlets~\cite{Jha&2015}, and can be adapted to $k=5$ by using sampling strategies for trees on five nodes~\cite{Wang&2015,Wang&2016}.
However, this technique does not give tight guarantees, and it is unclear how to scale it to $k>5$.
In contrast, here we aim at counting graphlets of size $k > 5$ with provable guarantees.

\item \textbf{Random walks.} These algorithms simulate a properly designed random walk over the graphlet occurrences in the host graph.
Standard random walk theory then says one can take unbiased graphlet samples after the chain mixes.
The first algorithm, GUISE~\cite{Bhuiyan&2012}, collected samples of $4$ and $5$-graphlets in graphs with a few million nodes in minutes -- a significant advancement of the state of the art at the time.
Further extensions and refinements followed~\cite{Wang&2014,Chen&2016,Han&2016}, confirming the prowess of the technique for $k \le 5$.
However,~\cite{Bressan&2017} showed that such approaches need $\Omega(n^{k-1})$ simulation steps even to hit one of the graphlets that form a $1-o(1)$ fraction of all occurrences.
Furthermore, deciding when to stop the random walk is nontrivial.
% making this technique less appealing.

\item \textbf{Color coding.} A randomized technique introduced to estimate the counts of trees and tree-like graphlets.
Parallel and distributed algorithms based on color coding can scale to large graphs with dozens of millions of nodes~\cite{Zhao&2010,Slota&2013,Chakaravarthy&2016}, but so far only for graphlets of very specific types.
Recently,~\cite{Bressan&2017} showed color coding can be extended to estimate the relative frequency of $k$-graphlets, for $k=5$ on medium-large graphs and for $k=6,7$ on smaller graphs.
This paper is discussed in more detail below.
\end{itemize}

The present paper builds on the findings of~\cite{Bressan&2017}, which provided a first theoretical and experimental comparison between random walks and color coding for \emph{approximating the relative frequency of the most frequent graphlets}.
The paper suggested color coding could scale beyond the state of the art, i.e.\ to $k>5$ on graphs on millions of nodes.
In this paper we confirm that result and extend the techniques beyond the mere estimation of relative frequencies of top-occurring graphlets.
Thanks to our extension, we can also provide novel insights into the structure of large graphs.

Finally we note that, for $k$-cliques,~\cite{Jain&2017} provides a fast approximated counting algorithm that runs in minutes for $k=10$ on real graphs with millions of nodes.
Those techniques are hard to extend to counting other graphlets.
In contrast, here we count approximately the occurrences of \emph{any given graphlet}, not only cliques, for $k$ reaching up to $10$.

%A related problem is subgraph \emph{enumeration}, which is clearly at least as hard as (approximate) subgraph counting.
%Indeed, an overwiew of recent contributions to parallel and distributed subgraph enumeration makes clear that it is not a viable approach to our problem.
%\cite{Shao&2014} introduce PSgL, a parallel subgraph listing tool based on a careful load balancing.
%PSgL was ran on $28$ cluster nodes, and it took more than one hour to enumerate the occurrences of one specific $5$-graphlet on a network with less than $1$M nodes and $10$M edges.
%\cite{Lai&2015} give a distributed MapReduce algorithm, TwinTwigJoin, further improved in~\cite{Lai&2016} with SEED.
%Tested on a $15$-node cluster, SEED manages to enumerate the occurrences of a specific $6$-node graphlet in the \lj\ graph in more than $1.5$ hours; since there are $112$ graphlets on $6$ nodes, this could mean more than $7$ days of computation to obtain the (exact) distribution.
%A similar scenario holds for $5$-graphlets with more than $15$ minutes needed for a single graphlet, which means more than $5$ hours for the full distribution.
%\cite{Kim&2016} designs a subgraph enumeration algorithm that saves memory requirements and I/O operations, and can run on a single machine.
%To enumerate the \lj\ occurrences of one specific $5$-node graphlet it takes roughly $1.4$ days on a single machine and roughly $1$ day on a cluster; translates to the full distribution over the $21$ possible $5$-node graphlets this means respectively one month and 20 days.
%%Similarly, the $15$-node cluster used for TwinTwigJoin was not powerful enough to count all $5$-nodes cliques in graphs with more than $3.2$M nodes and $12.2$M edges.
%%In contrast, \motivo\ can produce accurate counts of \emph{all} $5$-node graphles on graphs with tens of millions on nodes within minutes on a modern high-end PC.
%

